YBa$_2$Cu$_3$O$_7$ Josephson diode operating as a high-efficiency ratchet

Using a focused He$^+$ beam for nanopatterning and writing of Josephson barriers we fabricated specially shaped Josephson junctions of in-line geometry in YBa$_2$Cu$_3$O$_7$ thin film microbridges with an asymmetry ratio of critical currents of opposite polarities (non-reciprocity ratio) $\approx 7$ at optimum magnetic field. Those Josephson diodes were subsequently used as ratchets to rectify an applied ac current into a dc voltage. We also demonstrate the operation of such a ratchet in the loaded regime, where it produces a nonzero dc output power and yields a thermodynamic efficiency of up to $75\,\mathrm{\%}$. The ratchet shows record figures of merit: an output dc voltage of up to $212\,\mathrm{\mu V}$ and an output power of up to $0.2\,\mathrm{nW}$. The device has an essential area $\approx 1\,\mathrm{\mu m^2}$. For rectification of quasistatic Gaussian noise, the figures of merit are more modest, however the efficiency can be as high as for the deterministic ac drives within some regimes. Since the device is based on YBa$_2$Cu$_3$O$_7$, it can operate at temperatures up to $\sim40\,\mathrm{K}$, where more noise is available for rectification.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\ia}{\textit{i.a.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\@\xspace}
\newcommand{\rhs}{r.h.s.\@\xspace}
%German versions:
\renewcommand{\dh}{d.h.\xspace}
\newcommand{\zB}{z.B.\xspace}
\newcommand{\ua}{u.a.\xspace}
\newcommand{\vgl}{vgl.\xspace}
\newcommand{\usw}{usw.\xspace}
\newcommand{\bzw}{bzw.\xspace}


\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[2][\,]{\ensuremath{#1\mathrm{#2}}}


% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed only for 2 vars
% \fracpii{f}{x}{y}
\newcommand{\fracpii}[3]{\displaystyle\frac{\partial^{2}#1}{\partial#2\partial#3}}
%mixed derivatives are not implemented yet :-(
\newcommand{\fracpmix}[3]{\displaystyle\frac{\partial^2#1}{\partial#2\partial#3}}
%ideally: \fracp*{f}{x^2,y,z} or \fracp*{f}{x,x,y,z}
%usage: \divp{f}{x} produces partial derivative df/dx.
%usage with optional argument: \divp[2]{f}{x} produces 2nd order partial derivative
\newcommand{\divp}[3][]{{\partial^{#1}#2}/{\partial#3^{#1}}}

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle_{#1}}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

\newcommand{\bra}[1]{\ensuremath{\left\langle #1\right|}\xspace}
\newcommand{\ket}[1]{\ensuremath{\left| #1\right\rangle}\xspace}
\newcommand{\braket}[1]{\ensuremath{\left\langle #1\right\rangle}\xspace}

%shorter braces:
\newcommand\braces[1]{\rbraces{#1}}
\newcommand\rbraces[1]{\ensuremath{\left( #1\right)}}
\newcommand\sbraces[1]{\ensuremath{\left[ #1\right]}}
\newcommand\fbraces[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand\tbraces[1]{\ensuremath{\left< #1\right>}}
\newcommand\abraces[1]{\ensuremath{\left| #1\right|}}
%braced frac
\newcommand\rbfrac[2]{\ensuremath{\left( \frac{#1}{#2}\right)}}
\newcommand\sbfrac[2]{\ensuremath{\left[ \frac{#1}{#2}\right]}}
\newcommand\fbfrac[2]{\ensuremath{\left\{\frac{#1}{#2}\right\}}}
\newcommand\tbfrac[2]{\ensuremath{\left< \frac{#1}{#2}\right>}}
\newcommand\abfrac[2]{\ensuremath{\left| \frac{#1}{#2}\right|}}

%3D vectors with comma-separated coords
%usage: \VEC(1,1,0)
\def\innervector(#1,#2,#3){\begin{matrix}#1\\#2\\#3\end{matrix}}
\def\VEC#1{\braces{\negthinspace\innervector(#1)}}
\def\sVEC#1{\sbraces{\innervector(#1)}}
\def\fVEC#1{\fbraces{\negthinspace\innervector(#1)}}
\def\aVEC#1{\abraces{\innervector(#1)}}
\def\AVEC#1{\abraces{\abraces{\innervector(#1)}}}


%%
%% Freq used math symbols
%%

%Special (Elliptic) fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
\newcommand{\asinh}{\mathop{\mathrm{Arsinh}}\nolimits}
\newcommand{\acosh}{\mathop{\mathrm{Arcosh}}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{Artanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}

\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\ceil}{\mathop{\mathrm{ceil}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}

%%
%% Complex numbers {
%%
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\arg}{\mathop{\mathrm{arg}}\nolimits}
%imaginary i and j
\newcommand{\ii}{\ensuremath{\mathrm{i}}}
%\newcommand{\ij}{\ensuremath{\mathrm{i}}}
%%}

%some symbols that should be Roman to stress that they are not (parts of)variables
\newcommand{\dd}{\ensuremath{\,\mathrm{d}}}
\newcommand{\ee}{\ensuremath{\mathrm{e}}\xspace}

%\newcommand{\O}{\mathop{\mathrm{O}}\nolimits} %of the order of
%\newcommand{\d}{\mathop{\mathrm{d}}} %d like in integrad dx, dy, dz

%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\LSAT}{(LaAlO$_3$)$_3$(Sr$_2$AlTaO$_6$)$_7$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}

%%%
%%% Frequently used physics notations
%%%

%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}



%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

\newcommand{\kB}{\ensuremath{k_\mathrm{B}}}
\newcommand{\kBT}{\ensuremath{k_\mathrm{B}T}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections
%usage and result for ShowCorrection=true/false:
%\new{text} blue/normal
%\old{text} red strikedout/hidden
%\note{text} gray/hidden

\RequirePackage{ifthen}
\RequirePackage{color}
\usepackage[normalem]{ulem}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections/notes macros
\newcommand{\new}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor[rgb]{0,0,1}{#1}}{#1}%
}
\newcommand{\old}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor[rgb]{1,0,0}{\sout{#1}}}{}%
}
\newcommand{\note}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor{gray}{#1}}{}
}%

%select hard references to make them noticable
\newcommand{\hardref}[1]{\textcolor{orange}{#1}}

%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

\def\spins#1{\ensuremath{\spn#1.}}
\def\spn#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \uparrow
  \else\if#1d
    \downarrow
  \else\if#1U
    \Uparrow
  \else\if#1D
    \Downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1h
    \leftrightarrow
  \else\if#1v
    \updownarrow
  \else\if#1_%
    \;\;
  \else\if#1,%
    \,
  \else\if#1;%
    \;
  \else\if#1|%
    \vdots%
  \else\if#1-%
    \hdots%
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro spins}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\spn
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}



